Robustness of momentum-indirect interlayer excitons in MoS2/WSe2 heterostructure against charge carrier doping

Monolayer transition-metal dichalcogenide (TMD) semiconductors exhibit strong excitonic effects and hold promise for optical and optoelectronic applications. Yet, electron doping of TMDs leads to the conversion of neutral excitons into negative trions, which recombine predominantly non-radiatively at room temperature. As a result, the photoluminescence (PL) intensity is quenched. Here we study the optical and electronic properties of a MoS2/WSe2 heterostructure as a function of chemical doping by Cs atoms performed under ultra-high vacuum conditions. By PL measurements we identify two interlayer excitons and assign them to the momentum-indirect Q-Gamma and K-Gamma transitions. The energies of these excitons are in a very good agreement with ab initio calculations. We find that the Q-Gamma interlayer exciton is robust to the electron doping and is present at room temperature even at a high charge carrier concentration. Submicrometer angle-resolved photoemission spectroscopy (micro-ARPES) reveals charge transfer from deposited Cs adatoms to both the upper MoS2 and the lower WSe2 monolayer without changing the band alignment. This leads to a small (10 meV) energy shift of interlayer excitons. Robustness of the momentum-indirect interlayer exciton to charge doping opens up an opportunity of using TMD heterostructures in light-emitting devices that can work at room temperature at high densities of charge carriers.

==> Refs.tex <==
type-II band alignment provides a spatial separation of electrons and holes. 

In addition, the neutral excitons do not interact strongly with the charged defects.~\cite{Lien468}  

Excitons are already quenched in heterostructure due to the charge transfer:
https://pubs.acs.org/doi/pdf/10.1021/acsnano.5b02144

The multiple pathways: electron transfer, hole transfer, energy transfer, and Auger recombination.

where electron is photoexcited into K point, forming trion with two electrons in K-point and hole in Q-point.   

In addition - Cs adatoms - charged defects seems like not affect the scattering of charge neutral ILE = can be used in optoelectronics.

exciton-exciton annihilation through a

"result of competition between charge screening that destabilizes both
excitons and trions, and charge accumulation that is needed for
trions but not for excitons" (https://pubs.acs.org/doi/pdf/10.1021/nl4011172)

As a dopant we use Cs 
This imply that ILE1 and ILE2 peaks are indeed two distinct excitonic states. 

local minima in conduction band at the Q point 
Experiments at room temperature (at cryogenic temperatures the trions are pronounced)
To on 

Indirect exciton nature was demonstrated particularly by the fact that they disappear at low temperature (and trions appear), since the formation of these indirect excitons requrere phonon 

Scattering of electrons between K and Q valleys via optical phonons: (phonon-assisted scattering) https://www.nature.com/articles/s41699-017-0035-1.pdf
https://www.nature.com/articles/ncomms14670

 
In contrast to the K-points, the states in G and Q points "experience significant interlayer hybridization" 

Note, that hBN interlayer is essential to observe the PL - charge transfer to the graphene. Interestingly, on in a heterostructure on graphene region (marked by a star) we do not observe WSe2 PL. This might be related to the charge and energy transfer to graphene substrate.~\cite{Froehlicher_PRX}

the part of the TMD heterostructure on gr/SiC, which prevents the charging during the photoemission process.

Eneregy: indirect excitons as phonon replicas: 
https://www.nature.com/articles/s41467-018-04877-3

Spin polarization: https://arxiv.org/ftp/arxiv/papers/2006/2006.01970.pdf
https://arxiv.org/ftp/arxiv/papers/1701/1701.02770.pdf

Gamma-point variation with twist angle: https://www.hzdr.de/publications/PublDoc-14311.pdf

Trions: https://www.nature.com/articles/s41467-017-02286-6

large built-in interfacial electric field in heterobilayers: https://pubs.acs.org/doi/pdf/10.1021/acs.nanolett.7b03667

exciton binding enegy may vary from valley to valley (https://www.nature.com/articles/s41567-018-0123-y)

Momentum-dark excitons - Hogele (https://www.nature.com/articles/s41467-018-04877-3)

//Auger recombination rate increases with T: https://www.nature.com/articles/srep18885

Temperature-dependence of excitons and trions: https://journals.aps.org/prb/pdf/10.1103/PhysRevB.94.165301

Doping by K~\cite{Eknapakul2014} and Rb~\cite{Kang2017, Kim2017} (charge carrier concentration). Rb + K low temp~\cite{Riley2015}, WSe2 on hBN with K~\cite{Katoch2018}

